Understanding Children's Avatar Making in Social Online Games

Social online games like Minecraft and Roblox have become increasingly integral to children's daily lives. Our study explores how children aged 8 to 13 create and customize avatars in these virtual environments. Through semi-structured interviews and gameplay observations with 48 participants, we investigate the motivations behind children's avatar-making. Our findings show that children's avatar creation is motivated by self-representation, experimenting with alter ego identities, fulfilling social needs, and improving in-game performance. In addition, designed monetization strategies play a role in shaping children's avatars. We identify the ''wardrobe effect,'' where children create multiple avatars but typically use only one favorite consistently. We discuss the impact of cultural consumerism and how social games can support children's identity exploration while balancing self-expression and social conformity. This work contributes to understanding how avatar shapes children's identity growth in social online games.

==> altText/Alt_Text.tex <==
Figure 1: An image board displaying a variety of avatars created by children. The top row features avatars from the game Roblox, while the first three avatars on the bottom left are from Minecraft, and the rest are also from Roblox. This figure showcases the diversity in avatar customization choices made by children across different games.

Figure 2: Screenshot of Roblox’s Avatar Editor interface, where children can customize their characters. The interface shows options for clothing, accessories, head & body, and animation customization. Various items are displayed, some marked with a small coin icon indicating that they require in-game currency, Robux, to purchase.

Figure 3: Three avatars created by child participants to represent themselves in social games. From left to right, the avatars are designed by participants P250, P59, and P222. This figure illustrates the unique ways children use avatars to portray their identities in virtual environments.

Figure 4: Close-up screenshot of avatars, featuring various avatars from Roblox, surrounded by various customization options for head accessories. The available items range from basic hats to elaborate headgear.

Figure 5: An image showing a child participant’s avatar looks like two boxes stacked together, designed to improve camouflage and strength. 

Figure 6: Screenshot of Minecraft's avatar customization interface, displaying a range of clothing options. The top-left section shows "Featured Tops," which are paid items and are visually more attractive and decorative. The middle section, "Owned Tops," contains free items that are plain and less decorated. The lower rows show additional paid items under "All Tops."

Figure 7 Alt Text: Screenshot of a child participant's avatar library featuring various branded and culturally relevant characters such as Gandalf, Thanos, and Saruman. The figure highlights the influence of popular culture on children's choices for avatar customization in online games.
